Layered controller synthesis for dynamic multi-agent systems

In this paper we present a layered approach for multi-agent control problem, decomposed into three stages, each building upon the results of the previous one. First, a high-level plan for a coarse abstraction of the system is computed, relying on parametric timed automata augmented with stopwatches as they allow to efficiently model simplified dynamics of such systems. In the second stage, the high-level plan, based on SMT-formulation, mainly handles the combinatorial aspects of the problem, provides a more dynamically accurate solution. These stages are collectively referred to as the SWA-SMT solver. They are correct by construction but lack a crucial feature: they cannot be executed in real time. To overcome this, we use SWA-SMT solutions as the initial training dataset for our last stage, which aims at obtaining a neural network control policy. We use reinforcement learning to train the policy, and show that the initial dataset is crucial for the overall success of the method.

==> Makefile <==
all:
	for auxfile in $$(ls *.aux); do \
	  if (grep -q "bibstyle" $${auxfile} && \
	      grep -q "citation" $${auxfile}); then \
	    bibtex $${auxfile} || sleep 1; \
	  fi; \
	done; \
	pdflatex main.tex

main.pdf: main.tex
	pdflatex main.tex
	for auxfile in $$(ls *.aux); do \
	  if (grep -q "bibstyle" $${auxfile} && \
	      grep -q "citation" $${auxfile}); then \
	    bibtex $${auxfile} || sleep 1; \
	  fi; \
	done; \
	grep -q "Rerun to get" main.aux && pdflatex main.tex || true
	grep -q "Rerun to get" main.aux && pdflatex main.tex || true

latex-clean: emacs-clean
	for file in $$(ls *.tex) ; \
	  do \
	    base=`basename $${file} .tex` && \
	    (grep -q "\\documentclass" $${file} && \
	    for ext in log aux out bbl blg out vtc idx ilg ind thm nav toc snm tns cb cb2; \
	      do rm -f $${base}.$${ext}; \
	    done) || true; \
	  done; \
	for file in $$(ls *.log) ; do \
	  base=`basename $${file} .log` && \
	  (grep -q "/$${base}.tex" $${file} && \
	    for ext in log aux out bbl blg out vtc idx ilg ind thm nav toc snm tns; \
	      do rm -f $${base}.$${ext}; \
	    done) || true; \
	  done;
	(grep -q "bibunit" *tex && rm -f bu?.aux bu?.blg bu?.bbl) || true


==> sections/implementation.tex <==
\begin{itemize}
    \item Link to our github 
    \item Link to the notebook ? whatever making a simulation ? An example of nine cars sharing a path.
\end{itemize}
